ZTF SN~Ia DR2: Cosmology-independent constraints on Type Ia supernova standardisation from supernova siblings

Understanding Type Ia supernovae (SNe~Ia) and the empirical standardisation relations that make them excellent distance indicators is vital to improving cosmological constraints. SN~Ia ``siblings", i.e. two or more SNe~Ia in the same host or parent galaxy offer a unique way to infer the standardisation relations and their diversity across the population. We analyse a sample of 25 SN~Ia pairs, observed homogeneously by the Zwicky Transient Factory (ZTF) to infer the SNe~Ia light curve width-luminosity and colour-luminosity parameters $\alpha$ and $\beta$. Using the pairwise constraints from siblings, allowing for a diversity in the standardisation relations, we find $\alpha = 0.218 \pm 0.055 $ and $\beta = 3.084 \pm 0.312$, respectively, with a dispersion in $\alpha$ and $\beta$ of $\leq 0.195$ and $\leq 0.923$, respectively, at 95$\%$ C.L. While the median dispersion is large, the values within $\sim 1 \sigma$ are consistent with no dispersion. Hence, fitting for a single global standardisation relation, we find $\alpha = 0.228 \pm 0.029 $ and $\beta = 3.160 \pm 0.191$. We find a very small intrinsic scatter of the siblings sample $\sigma_{\rm int} \leq 0.10$ at 95\% C.L. compared to $\sigma_{\rm int} = 0.22 \pm 0.04$ when computing the scatter using the Hubble residuals without comparing them as siblings. Splitting the sample based on host galaxy stellar mass, we find that SNe~Ia in both subsamples have consistent $\alpha$ and $\beta$. The $\beta$ value is consistent with the value for the cosmological sample. However, we find a higher $\alpha$ by $\sim 2.5 - 3.5 \sigma$. The high $\alpha$ is driven by low $x_1$ pairs, potentially suggesting that the slow and fast declining SN~Ia have different slopes of the width-luminosity relation. We can confirm or refute this with increased statistics from near future time-domain surveys. (abridged)

==> tables/des_siblings_parameters.tex <==
\begin{table*}
\caption{SALT2 fit parameters, using the FPBot photometry for all the sibling pairs analysed in this study \sdt{same as above but with FPBot, keeping both copies for now till the sample is finalised}}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
SN1 & z & $m_B$-1 & $x_1$-1 & $c$-1 & SN2 &  $m_B$-2 & $x_1$-2 & $c$-2 \\
\hline 

DES13S2dlj & DES14S2pkz & 0.229 & 21.902 +/- 0.035 & 21.378 +/- 0.031 & 0.526 +/- 0.234 & -0.484 +/- 0.125 & 0.209 +/- 0.027 & 0.075 +/- 0.027 \\
DES14C3zym & DES15C3edd & 0.36 & 22.309 +/- 0.028 & 22.464 +/- 0.03 & -1.576 +/- 0.124 & -1.363 +/- 0.149 & -0.084 +/- 0.024 & -0.05 +/- 0.024 \\
DES14C2iku & DES17C2jjb & 0.384 & 24.628 +/- 0.197 & 22.546 +/- 0.041 & 1.748 +/- 1.798 & -0.607 +/- 0.277 & 0.662 +/- 0.152 & 0.009 +/- 0.152 \\
DES15S2okk & DES17S2alm & 0.507 & 22.89 +/- 0.047 & 23.223 +/- 0.064 & 1.921 +/- 1.178 & 3.088 +/- 0.927 & -0.013 +/- 0.038 & 0.017 +/- 0.038 \\
DES15C2mky & DES16C2cqh & 0.525 & 22.913 +/- 0.04 & 23.602 +/- 0.127 & 0.968 +/- 0.357 & 2.583 +/- 1.404 & -0.067 +/- 0.034 & 0.036 +/- 0.034 \\
DES13E1wu & DES14E1uti & 0.561 & 23.108 +/- 0.059 & 23.312 +/- 0.076 & 1.041 +/- 0.941 & 3.612 +/- 2.397 & -0.018 +/- 0.046 & -0.026 +/- 0.046 \\
DES16C3nd_1 & DES16C3nd_2 & 0.648 & 23.805 +/- 0.034 & 23.64 +/- 0.031 & -0.717 +/- 0.318 & 0.007 +/- 0.285 & 0.023 +/- 0.037 & 0.058 +/- 0.037 \\
DES15X2mlr & DES15X2nku & 0.649 & 23.424 +/- 0.068 & 23.899 +/- 0.089 & -0.439 +/- 0.77 & 3.172 +/- 1.445 & -0.117 +/- 0.059 & -0.023 +/- 0.059 \\

\hline
\end{tabular}
\label{tab:des_sne}
\end{table*}

==> tables/final_sibling_photsample.tex <==
\begin{table*}
\caption{SALT2 fit parameters for the sample with one spectroscopic SN~Ia and one photometric SN~Ia siblings pair, i.e. the "phot-spec" subsample.}
\resizebox{.95\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
SN1 &  SN2 & Ang. Sep (``) z & $m_B$-1 &  $m_B$-2 & $x_1$-1   & $x_1$-2 & $c$-1 & $c$-2 &  log Mass (log $M_{\odot}$) \\
\hline
ZTF19acbzdvp_1 & ZTF19acbzdvp_2 & 0.0 & 0.103 & 19.403 +/- 0.037 & 19.115 +/- 0.039 & -0.286 +/- 0.211 & -1.141 +/- 0.432 & 0.114 +/- 0.03 & 0.007 +/- 0.03 &10.05 \\
ZTF19aambfxc_1 & ZTF19aambfxc_2 & 0.0 & 0.0541 & 19.878 +/- 0.061 & 17.531 +/- 0.033 & 0.471 +/- 0.28 & 0.222 +/- 0.128 & 0.741 +/- 0.044 & -0.01 +/- 0.044 &10.33 \\
%ZTF20aamibse_1 & ZTF20aamibse_2 & 0.0 & 0.097 & 20.083 +/- 0.143 & 19.177 +/- 0.082 & -0.736 +/- 1.9 & -0.71 +/- 0.81 & 0.469 +/- 0.096 & -0.097 +/- 0.096 &10.4 \\
ZTF19abaeyln & ZTF20abeadnl & 2.3 & 0.0852 & 18.585 +/- 0.039 & 19.488 +/- 0.049 & 0.401 +/- 0.277 & -1.73 +/- 0.301 & 0.129 +/- 0.032 & 0.119 +/- 0.032 &10.6 \\
ZTF20abazgfi & ZTF19acgemxh & 2.5 & 0.09 & 18.849 +/- 0.036 & 19.93 +/- 0.055 & 0.184 +/- 0.157 & -0.614 +/- 0.811 & 0.046 +/- 0.031 & 0.358 +/- 0.031 &10.36 \\
ZTF20abgaovd & ZTF19abtuhqa & 2.7 & 0.1 & 18.521 +/- 0.054 & 18.29 +/- 0.044 & -0.901 +/- 0.335 & 0.296 +/- 0.414 & 0.02 +/- 0.045 & 0.019 +/- 0.045 &10.66 \\
ZTF18aakaljn & ZTF19acdtmwh & 3.0 & 0.0699 & 18.348 +/- 0.049 & 18.993 +/- 0.064 & 1.524 +/- 0.342 & -0.503 +/- 0.398 & 0.139 +/- 0.043 & 0.217 +/- 0.043 &10.9 \\
ZTF22aaksdvi & ZTF21acowrme & 7.9 & 0.0821 & 18.308 +/- 0.031 & 18.668 +/- 0.06 & -0.255 +/- 0.123 & 1.151 +/- 1.04 & -0.109 +/- 0.026 & -0.047 +/- 0.026 &10.84 \\
ZTF18abuiknd & ZTF20acqpzbo & 8.6 & 0.104 & 19.089 +/- 0.033 & 18.959 +/- 0.045 & 0.452 +/- 0.268 & 0.873 +/- 0.327 & -0.03 +/- 0.03 & -0.003 +/- 0.03 &10.75 \\
ZTF20abgfvav & ZTF18abktzep & 9.1 & 0.095 & 19.117 +/- 0.035 & 19.906 +/- 0.056 & 0.074 +/- 0.193 & 0.112 +/- 0.624 & 0.038 +/- 0.03 & 0.24 +/- 0.03 &9.59 \\
ZTF19aatzlmw & ZTF20aaznsyq & 11.0 & 0.073 & 18.342 +/- 0.074 & 18.326 +/- 0.044 & -0.183 +/- 0.351 & -0.348 +/- 0.17 & -0.031 +/- 0.051 & -0.013 +/- 0.051 &10.73 \\
ZTF21aajfpwk & ZTF19aacxwfb & 17.8 & 0.0791 & 18.993 +/- 0.03 & 18.865 +/- 0.037 & -2.248 +/- 0.107 & -2.092 +/- 0.205 & -0.003 +/- 0.025 & -0.037 +/- 0.025 &11.38 \\
ZTF18aaqcozd & ZTF19aaloezs & 21.1 & 0.073 & 18.451 +/- 0.031 & 18.801 +/- 0.032 & -1.324 +/- 0.107 & -2.165 +/- 0.081 & -0.094 +/- 0.026 & 0.011 +/- 0.026 &10.87  \\
ZTF20abrgyhd & ZTF19aatvlbw & 30.1 & 0.066 & 18.447 +/- 0.031 & 19.077 +/- 0.043 & -1.918 +/- 0.107 & -2.264 +/- 0.207 & -0.012 +/- 0.027 & 0.16 +/- 0.027 &11.1 \\
\hline
\end{tabular}}
\label{tab:saltparams_phot}
\end{table*}

==> tables/final_sibling_specsample.tex <==
\begin{table}
\caption{List of SNe in the spectroscopic Ia siblings sample}
\begin{tabular}{|c|c|}
\hline 
SN$_1$ & SN$_2$ \\
\hline
Spec \\
ZTF18abnucig & ZTF20achyvas \\
ZTF22abveefy & ZTF21abnfdqg \\
ZTF20acehyxd & ZTF21abouuow \\
ZTF20aaeszsm & ZTF20abujoya \\
ZTF20abptxls & ZTF21aabpszb \\
ZTF20aaxicpu & ZTF21abasxdp \\
ZTF19aaugoig & ZTF22abmzete \\
ZTF19accobqx & ZTF19acnwelq \\
ZTF20abatows & ZTF20abcawtk \\
ZTF22abanxam & ZTF20aasctts \\
ZTF20abydkrl & ZTF20acpmgdz \\
ZTF19abjpkdz & ZTF19aculypc \\
ZTF18abdmgab & ZTF20abqefja \\
\hline 
Photo-Spec \\
\hline
\end{tabular}
\end{table}


==> tables/salt_params.tex <==
\begin{table*}
\caption{SALT2 fit parameters for all the sibling pairs analysed in this study \sdt{clean up table with FPBot?}}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
SN1 & z & $m_B$-1 & $x_1$-1 & $c$-1 & SN2 &  $m_B$-2 & $x_1$-2 & $c$-2 \\
\hline
ZTF20abatows & 0.0945 & 19.1042 $\pm$ 0.051 & 0.01 $\pm$ 0.36 & 0.03 $\pm$ 0.04 & ZTF20abcawtk & 19.1035 $\pm$ 0.041 & -0.86 $\pm$ 0.22 & -0.04 $\pm$ 0.04 \\ 
ZTF20abbhyxu & 0.0319 & 16.4655 $\pm$ 0.038 & -0.56 $\pm$ 0.1 & 0.04 $\pm$ 0.03 & ZTF20acebweq & 16.83 $\pm$ 0.767 & -1.46 $\pm$ 6.62 & 0.15 $\pm$ 0.45 \\ 
ZTF18abnucig & 0.09 & 18.8574 $\pm$ 0.089 & 0.46 $\pm$ 0.64 & -0.03 $\pm$ 0.07 & ZTF20achyvas & 18.7326 $\pm$ 0.064 & 1.58 $\pm$ 0.93 & -0.11 $\pm$ 0.08 \\ 
ZTF20acehyxd & 0.035 & 18.1299 $\pm$ 0.099 & 0.21 $\pm$ 0.61 & 0.41 $\pm$ 0.07 & ZTF21abouuow & 16.537 $\pm$ 0.037 & 0.74 $\pm$ 0.1 & 0.02 $\pm$ 0.03 \\ 
ZTF19abjpkdz & 0.0564 & 18.9834 $\pm$ 0.095 & -3.48 $\pm$ 1.4 & 0.16 $\pm$ 0.07 & ZTF19aculypc & 17.5706 $\pm$ 0.086 & -1.15 $\pm$ 0.32 & -0.04 $\pm$ 0.06 \\ 
ZTF20aaeszsm & 0.07 & 18.5923 $\pm$ 0.052 & 0.26 $\pm$ 0.55 & 0.11 $\pm$ 0.04 & ZTF20abujoya & 18.6639 $\pm$ 0.086 & -1.38 $\pm$ 0.54 & 0.05 $\pm$ 0.06 \\ 
ZTF20abptxls & 0.0163 & 15.1709 $\pm$ 0.035 & 0.78 $\pm$ 0.08 & 0.07 $\pm$ 0.03 & ZTF21aabpszb & 15.4641 $\pm$ 0.043 & -0.49 $\pm$ 0.09 & 0.03 $\pm$ 0.03 \\ 
 ZTF20aaxicpu & 0.0721 & 18.6525 $\pm$ 0.055 & -1.42 $\pm$ 0.31 & -0.07 $\pm$ 0.05 & ZTF21abasxdp & 18.6261 $\pm$ 0.04 & -1.52 $\pm$ 0.22 & 0.01 $\pm$ 0.03 \\ 
ZTF20abydkrl & 0.0311 & 16.5545 $\pm$ 0.042 & -0.95 $\pm$ 0.1 & 0.05 $\pm$ 0.03 & ZTF20acpmgdz & 16.4707 $\pm$ 0.033 & -0.31 $\pm$ 0.05 & 0.05 $\pm$ 0.03 \\ 
ZTF18adaadmh & 0.0445 & 17.5819 $\pm$ 0.045 & 0.54 $\pm$ 0.44 & 0.02 $\pm$ 0.04 & ZTF20aamujvi & 17.7679 $\pm$ 1.404 & -10.4 $\pm$ 222.27 & -0.31 $\pm$ 3.43 \\ 
ZTF22abanxam & 0.0457 & 18.547 $\pm$ 0.052 & -2.82 $\pm$ 0.63 & 0.19 $\pm$ 0.05 & ZTF20aasctts & 17.473 $\pm$ 0.059 & 1.05 $\pm$ 0.26 & 0.06 $\pm$ 0.04 \\ 
\hline
\end{tabular}
\label{tab:saltparams}
\end{table*}


==> tables/summary_salt_selection.tex <==
\begin{table*}
\caption{SALT2 fit parameters, using the FPBot photometry for all the photometric sibling pairs \sdt{aim is to have the parameters for the selection function}}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
SN-1 & $x_1$ & $\sigma(x_1)$ & $c$ & $\sigma(c)$ & Phase g & Phase r & SN-2 & $x_1$ & $\sigma(x_1)$ & $c$ & $\sigma(c)$ & Phase g & Phase r \\
\hline
ZTF20aagnbpw & 1.2473 & 0.0418 & 0.824 & 0.0278 & -12.7564 & -14.8155 & ZTF20aaunioz & 4.2697 & 0.4083 & 0.7635 & 0.0357 & -62.4266 & -67.5301 \\
ZTF20abjnmhn & 2.0264 & 0.1038 & -0.1073 & 0.0311 & -16.1174 & -774.0328 & ZTF20aaqshsc & -1.3616 & 0.3895 & -0.0834 & 0.0335 & -8.266 & -644.4724 \\
ZTF19abaeyln & 0.9854 & 0.0901 & 0.1108 & 0.0297 & -10.8568 & -14.8535 & ZTF20abeadnl & -0.4918 & 0.0787 & 0.1391 & 0.03 & -10.7408 & -537.4718 \\
ZTF20abazgfi & -0.0896 & 0.0497 & 0.0241 & 0.0288 & -268.7537 & -668.7217 & ZTF19acgemxh & 0.2028 & 0.168 & 0.3832 & 0.0323 & -4.1246 & -404.0519 \\
ZTF20abgaovd & -0.5145 & 0.099 & -0.0019 & 0.0317 & -304.4909 & -15.3892 & ZTF19abtuhqa & 0.5462 & 0.12 & -0.0039 & 0.0317 & -13.4898 & -13.4986 \\
ZTF20aaznlnj & -1.1697 & 0.0574 & -0.0836 & 0.0276 & -758.2247 & -704.2673 & ZTF19aaklsto & 0.4551 & 0.0426 & -0.0147 & 0.027 & -305.3633 & -224.5901 \\
ZTF18aakaljn & 0.1492 & 0.1109 & 0.3396 & 0.0306 & 0.8485 & -12.1311 & ZTF19acdtmwh & -0.2362 & 0.1002 & 0.1778 & 0.029 & -9.6069 & -342.584 \\
ZTF21aaxvrva & 1.1624 & 0.0734 & 0.5326 & 0.0298 & -4.9731 & -859.7976 & ZTF21abhqoja & -0.1409 & 0.0539 & 0.3191 & 0.0299 & -1.2887 & -1115.2396 \\
ZTF21aajfpwk & -1.3755 & 0.035 & 0.0381 & 0.0275 & -12.7128 & -13.6293 & ZTF19aacxwfb & -2.224 & 0.0748 & 0.023 & 0.0274 & -10.9947 & -10.0591 \\
ZTF18abzpbpi & 0.2659 & 0.0602 & 0.1596 & 0.0296 & -11.6592 & -8.6471 & ZTF21aaletht & -0.3019 & 0.0461 & 0.0968 & 0.0284 & -10.0006 & -15.0302 \\
ZTF19aaksrgj & 1.1543 & 0.0656 & 0.0018 & 0.0291 & -10.5858 & -36.407 & ZTF20aavpwxl & 0.1573 & 0.0978 & 0.127 & 0.0301 & -349.7499 & -373.6215 \\
ZTF20abgfvav & 0.0615 & 0.0455 & 0.0489 & 0.0292 & -13.6872 & -13.711 & ZTF18abktzep & -0.88 & 0.09 & 0.2878 & 0.0305 & -8.1946 & -8.2496 \\
ZTF21aagkvqa & -0.2879 & 0.1068 & -0.4207 & 0.0336 & 19.3342 & 19.3159 & ZTF20abhttyd & 1.0231 & 0.0765 & 0.4572 & 0.031 & -1.819 & -11.7297 \\
ZTF19aatzlmw & 0.1896 & 0.1061 & -0.0297 & 0.0303 & -7.7461 & -10.7282 & ZTF20aaznsyq & -0.3449 & 0.0632 & -0.0269 & 0.0293 & -13.7977 & -0.8616 \\
ZTF19aakluwr & -0.2368 & 0.5466 & 0.0512 & 0.0495 & -212.6355 & -7.0078 & ZTF20acpqbue & -2.2026 & 0.1217 & -0.0381 & 0.0499 & -822.0997 & -494.1132 \\
ZTF18aaqcozd & -1.2689 & 0.0424 & -0.0786 & 0.0272 & -11.2572 & -11.2083 & ZTF19aaloezs & -1.7942 & 0.0324 & 0.0552 & 0.0272 & -7.9641 & -332.9846 \\
ZTF20abrgyhd & -1.5068 & 0.04 & 0.0117 & 0.0274 & -9.9729 & -589.2135 & ZTF19aatvlbw & -2.1937 & 0.1369 & 0.16 & 0.0368 & -8.1913 & -122.5642 \\
ZTF20abasewu & -1.9001 & 0.0545 & -0.247 & 0.0312 & 51.7243 & -8.2714 & ZTF20acdccnl & -3.0463 & 0.2128 & 0.3791 & 0.0287 & -9.3683 & -10.4206 \\
ZTF20acmgkqe & 5622.7128 & 43.4541 & -0.017 & 0.0002 & -292.5287 & -724.4033 & ZTF17aadlxmv & 0.4275 & 0.0403 & 0.0766 & 0.0283 & -13.8282 & -446.5128 \\
ZTF18aazcoob & 0.7141 & 0.0326 & 0.0412 & 0.0262 & -16.7082 & -16.7715 & ZTF19aalbqxs & 0.2881 & 0.1011 & 0.0037 & 0.0295 & -5.8262 & -5.7335 \\
ZTF18abuiknd & 0.8556 & 0.1043 & -0.0075 & 0.0299 & -15.9122 & -14.8842 & ZTF20acqpzbo & 1.7125 & 0.0827 & 0.0174 & 0.03 & -475.1329 & -826.2351 \\
ZTF22aaksdvi & -0.4922 & 0.0415 & -0.1192 & 0.0283 & -12.1502 & -1090.1088 & ZTF21acowrme & -0.1759 & 0.1582 & -0.0162 & 0.0291 & -14.1124 & -345.1546 \\


\hline
\end{tabular}
\label{tab:summary_sample}
\end{table*}
